Where Did the Web Archive Go?

To perform a longitudinal investigation of web archives and detecting variations and changes replaying individual archived pages, or mementos, we created a sample of 16,627 mementos from 17 public web archives. Over the course of our 14-month study (November, 2017 - January, 2019), we found that four web archives changed their base URIs and did not leave a machine-readable method of locating their new base URIs, necessitating manual rediscovery. Of the 1,981 mementos in our sample from these four web archives, 537 were impacted: 517 mementos were rediscovered but with changes in their time of archiving (or Memento-Datetime), HTTP status code, or the string comprising their original URI (or URI-R), and 20 of the mementos could not be found at all.

==> cuts.tex <==

\section{Introduction}

(1) Library and Archives Canada (\url{collectionscanada.gc.ca})
Around May 2018, mementos in this archive were moved to a new archive (\url{webarchive.bac-lac.gc.ca}) which has a different domain name. We noticed that 49 mementos (out of 351) can not be found in the new archive.

(2) The National Library of Ireland (NLI) 
Around May 2018, the European Archive (\url{europarchive.org}) was shut down and the domain name was purchased by another entity. The National Library of Ireland (NLI) collection preserved by this archive was moved to another archive (\url{internetmemory.org}). All 979 mementos can be retrieved from the new archive (i.e., no missing mementos). Around September 2018, the archive internetmemory.org became unreachable (timeout error). The NLI collection preserved by this archive was moved to another archive (\url{archive-it.org}). The other archived collections in internetmemory.org may also have been moved to archive-it.org or to other archives. The number of missing from NLI mementos is 192 (out of 979).

(3) Public Record Office of Northern Ireland (PRONI) (\url{webarchive.proni.gov.uk})
Around October 2018, all mementos preserved by this archive were moved to archive-it.org. The PRONI archive's homepage  is still online and shows a list of web pages' URLs (not mementos' URLs). By clicking on any of these URLs, it redirects to an HTML page in archive-it.org that shows the available mementos (i.e., the TimeMap) associated with the selected URL. The number of missing mementos from PRONI is 114 (out of 469).

(4) Perma.cc

In this paper, we report on changes made to four web archives between May - October 2018.

(4) WebCite (\url{webcitation.org})
The archive has been unreachable (timeout error) for about a month (from June 06, 2019 to July 08, 2019). The archive no longer accepts any new archiving requests, but it still provides access to all preserved mementos.

\begin{table}
\centering
\caption{Web archives in our study, with total URI-Rs and URI-Ms observed. \todo{MAYBE DON'T NEED URI-Rs HERE?}}
\label{tab:archives}
\begin{tabular}{|l|r|r|}
\hline
\textbf{Web Archive} &  \textbf{URI-Rs} & \textbf{URI-Ms}\\ \hline
\url{web.archive.org} &  1,566 & 1,566\\
\url{archive-it.org} & 1,388 & 1,383\\
\url{archive.is}              & 1,257 & 1,396  \\
\url{webarchive.loc.gov}      & 1,059 & 1,594  \\
\url{arquivo.pt}              & 766   & 1,569  \\
\url{webcitation.org}         & 720   & 1,585  \\
\emph{\url{europarchive.org}}        & 321   & 979    \\
\url{swap.stanford.edu}       & 302   & 1,222  \\
\url{vefsafn.is}              & 290   & 1,589  \\
\url{webharvest.gov}          & 247   & 712    \\
\url{digar.ee}                & 225   & 488    \\
\url{webarchive.org.uk}       & 221   & 349    \\
\emph{\url{webarchive.proni.gov.uk}} & 209   & 469    \\
\url{nationalarchives.gov.uk} & 200   & 994    \\
\emph{\url{collectionscanada.gc.ca}} & 198   & 351    \\
\emph{\url{perma.cc}}                & 175   & 182    \\
\url{archive.bibalex.org}     & 168   & 199    \\ \hline
\textbf{Total}                   & \textbf{9,262} & \textbf{16,627} \\ \hline
\end{tabular}
\end{table}


\begin{table}
\centering
\caption{Web archives that changed during 2018}
\label{tab:archive-changes}
\begin{tabular}{|p{0.25\linewidth}|r|p{0.18\linewidth}|p{0.27\linewidth}|p{0.14\linewidth}|}
\hline
\textbf{Original Archive} & \textbf{URI-Ms} & \textbf{Date Change Discovered} & \textbf{New Archive} & \textbf{Missing Mementos} \\ \hline
LAC & & & & \\
{\scriptsize \url{collectionscanada.gc.ca}} & 351 & May 2018 & {\scriptsize \url{webarchive.bac-lac.gc.ca}} & 49 \\ \hline
NLI & & & & \\
{\scriptsize \url{europarchive.org}} & 979 & May 2018 & {\scriptsize \url{internetmemory.org}} & 0 \\ \hline
NLI & & & & \\
{\scriptsize \url{internetmemory.org}} & 979 & Sep 2018 & {\scriptsize \url{archive-it.org}} & 192 \\ \hline
PRONI & & & & \\
{\scriptsize \url{webarchive.proni.gov.uk}} & 469  & Oct 2018 & {\scriptsize \url{archive-it.org}} & 114 \\ \hline
\url{Perma.cc} & 182 & & & \\ \hline
\end{tabular}
\end{table}

%Table \ref{tab:findings} shows the summary of our observations for all four archives.
%\begin{table}
%\centering
%\caption{Observations about web archives that moved}
%\label{tab:findings}
%\begin{tabular}{|p{0.05\linewidth}|p{0.65\linewidth}|p{0.25\linewidth}|}
%\hline
% & \textbf{Finding} & \textbf{Archives Affected} \\ \hline
%1 & Old URI-M does not redirect to new archive & LAC, PRONI, NLI?, Perma.cc \\ \hline
%2 & Some mementos are missing & LAC, NLI, PRONI \\ \hline
%3 & HTTP status code may be different & LAC, NLI \\ \hline
%4 & Loss of functionality in new archive banner & NLI, PRONI \\ \hline
%5 & Original archive host no longer available & NLI \\ \hline
%6 & New archive handles HTTP 4xx/5xx status differently & NLI, PRONI \\ \hline
%7 & Some URI-Rs missing & PRONI \\ \hline
%\end{tabular}
%\end{table}

\section{Findings}

\subsection{Library and Archives Canada}

Figure \ref{fig:collectionscanada} shows a set of screenshots taken for the memento within 14 months. The screenshots with a blue border are representations of mementos in the original archive \url{www.collectionscanada.gc.ca}) before it is moved to the new archive. The screenshots with a red border is the home page of the new archive before we manually detected the corresponding URI-Ms in the new archive. The screenshots with a green border shows the representations resulting from requesting the memento from the new archive (\url{webarchive.bac-lac.gc.ca}). The representation before the archive's change (blue border) is different from the representation of the memento after the change (green border).
\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{figs/collectionscanada-thumbnails.png}
\caption{Screenshots of replaying the URI-M \url{TBD} 33 times over 14 months. The blue border indicates the presence in the original archive, red the unavailable mementos, and green the presence in the new archive.} 
\label{fig:collectionscanada}
\end{figure}


The representations of both mementos are illustrated in the figure below. The original archive uses the green banner (left) while the new archive uses the yellow banner (right):

\begin{lstlisting}
$ curl --head --location --silent http://www.collectionscanada.gc.ca/webarchives/20051228174058/http://nationalatlas.gov/ | egrep -i "(HTTP/1.1|^location:)"

Location: http://www.bac-lac.gc.ca/eng/discover/archives-web-government/Pages/web-archives.aspx
HTTP/1.1 302 Found
Location: http://webarchive.bac-lac.gc.ca/?lang=en
HTTP/1.1 200
\end{lstlisting}

Here is the representation of the home page of the new archive:


\begin{lstlisting}
$ curl --head --location --silent http://eot.us.archive.org/eot/20120520120841/http://www2.ed.gov/espanol/parents/academic/matematicas/brochure.pdf | egrep -i "(HTTP/|^location:)"

HTTP/1.1 302 Found
Location: https://web.archive.org/web/20120520120841/http://www2.ed.gov/espanol/parents/academic/matematicas/brochure.pdf
HTTP/2 200
\end{lstlisting}


\begin{lstlisting}
$ curl --head --location --silent http://webarchive.bac-lac.gc.ca:8080/wayback/20060208075019/http://www.cdc.gov/ | egrep -i "(HTTP/|^location:|^Memento-Datetime)"

HTTP/1.1 302 Found
Location: http://webarchive.bac-lac.gc.ca:8080/wayback/20061026060247/http://www.cdc.gov/
HTTP/1.1 200 OK
Memento-Datetime: Thu, 26 Oct 2006 06:02:47 GMT
\end{lstlisting}

If the original archive serves only mementos under /webarchives, then the mod\_rewrite rule would be even simpler:

\begin{lstlisting}
# With mod_rewrite
RewriteEngine on
RewriteRule   "^/webarchives/(.+)" http://webarchive.bac-lac.gc.ca:8080/wayback/$1  [L,R=301]
\end{lstlisting}

\paragraph{Observation 3: New features available in the new archive because of the upgraded replay tool}

The new archive (\url{webarchive.bac-lac.gc.ca}) uses an updated version of OpenWayback (i.e., OpenWayback Release 1.6.0 or later) that enables new features that were not supported by the original archive that was running OpenWayback Release 1.4 (or earlier):
\begin{itemize}
    \item \textbf{Raw Mementos.} Many archives allow accessing unaltered, or raw, archived content (i.e., retrieving the archived original content without any type of transformation by the archive). The most common mechanism to retrieve the raw mementos is by adding \texttt{id\_} after the timestamp in the requested URI-M. The feature of retrieving the raw mementos was not provided by the original archive. However, it is supported by the new archive. 
\item \textbf{Memento Support.} The new archive provides native support for the Memento protocol and returns Memento HTTP headers in the responses from the web archive. \todo{IS THIS CORRECT?}

\end{itemize}


\paragraph{Raw mementos}

At replay time, archives transform the original content of web pages to appropriately replay them (e.g., in a user’s browser). Archives add their own banners to provide metadata about both the memento being viewed and the original page. Archives also rewrite links of embedded resources in a page so that these resources are retrieved from the archive, not from the original server.

Many archives allow accessing unaltered, or raw, archived content (i.e., retrieving the archived original content without any type of transformation by the archive). The most common mechanism to retrieve the raw mementos is by adding \texttt{id\_} after the timestamp in the requested URI-M.

The feature of retrieving the raw mementos was not provided by the original archive (www.collectionscanada.gc.ca). However, it is supported by the new archive. For example, to retrieve the raw content of the memento identified by the URI-M

\url{http://webarchive.bac-lac.gc.ca:8080/wayback/20061026060247/http://www.cdc.gov/}

we add \texttt{id\_} after the timestamp as shown in the cURL session below:

\begin{lstlisting}
curl --head --location --silent http://webarchive.bac-lac.gc.ca:8080/wayback/20061026060247id_/http://www.cdc.gov/ | egrep -i "(HTTP/|^Memento-Datetime)"

HTTP/1.1 200 OK
Memento-Datetime: Thu, 26 Oct 2006 06:02:47 GMT
\end{lstlisting}

\paragraph{Memento Support}
The Memento protocol is supported by most public web archives including the Internet Archive. The protocol introduces two HTTP headers for content negotiation. First, Accept-Datetime is an HTTP Request header through which a client can request a prior state of a web resource by providing the preferred datetime, for example,

\begin{lstlisting}
Accept-Datetime: Mon, 09 Jan 2017 11:21:57 GMT.
\end{lstlisting}

Second, the Memento-Datetime HTTP Response header is sent by a server to indicate the datetime at which the resource was captured, for instance,

\begin{lstlisting}
Memento-Datetime: Sun, 08 Jan 2017 09:15:41 GMT.
\end{lstlisting}

The Memento protocol also defines:

\begin{itemize}
    \item TimeMap: A resource that provides a list of mementos (URI-Ms) for a particular original resource, 
\item TimeGate: A resource that supports content negotiation based on datetime to access prior versions of an original resource. 
\end{itemize}

The cURL session below shows the TimeMap of the original resource (\url{http://www.cdc.gov/}) available in the new archive. The TimeMap indicates that the memento with the Memento-Datetime Wed, 08 Feb 2006 07:50:19 GMT (as described above) is not available in the new archive.

\begin{lstlisting}
$ curl http://webarchive.bac-lac.gc.ca:8080/wayback/timemap/link/http://www.cdc.gov/

<http://www.cdc.gov/>; rel="original",
<http://webarchive.bac-lac.gc.ca:8080/wayback/timemap/link/http://www.cdc.gov/>; rel="self"; type="application/link-format"; from="Thu, 26 Oct 2006 06:02:47 GMT"; until="Fri, 09 Oct 2015 13:26:42 GMT",
<http://webarchive.bac-lac.gc.ca:8080/wayback/http://www.cdc.gov/>; rel="timegate",
<http://webarchive.bac-lac.gc.ca:8080/wayback/20061026060247/http://www.cdc.gov/>; rel="first memento"; datetime="Thu, 26 Oct 2006 06:02:47 GMT",
<http://webarchive.bac-lac.gc.ca:8080/wayback/20151009132642/http://www.cdc.gov/>; rel="last memento"; datetime="Fri, 09 Oct 2015 13:26:42 GMT"
\end{lstlisting}

It is possible that two archives use the same version of OpenWayback but with different configuration options, such as whether to support Memento framework or not:

\begin{lstlisting}
 <bean name="standardaccesspoint" class="org.archive.wayback.webapp.AccessPoint">
  <property name="accessPointPath" value="${wayback.url.prefix}/wayback/"/>
  <property name="internalPort" value="${wayback.url.port}"/>
  <property name="serveStatic" value="true" />
  <property name="bounceToReplayPrefix" value="false" />
  <property name="bounceToQueryPrefix" value="false" />
  <property name="enableMemento" value="true" />
\end{lstlisting}

or how to respond to (raw) archival redirects (thanks to Alex Osborne for help in locating this information):

\begin{lstlisting}
<!-- WARN CLIENT ABOUT PATH REDIRECTS -->
<bean class="org.archive.wayback.replay.selector.RedirectSelector">
 <property name="renderer">
   <bean class="org.archive.wayback.replay.JSPReplayRenderer">
     <property name="targetJsp" value="/WEB-INF/replay/UrlRedirectNotice.jsp" />
   </bean>
 </property>
</bean>
...
<!-- Explicit (via "id_" flag) IDENTITY/RAW REPLAY -->
<bean class="org.archive.wayback.replay.selector.IdentityRequestSelector">
  <property name="renderer" ref="identityreplayrenderer"/>
</bean>
\end{lstlisting}

\subsubsection{Summary}

When Library and Archives Canada migrated their archive in May 2018, 49 of the 351 mementos we were tracking resurfaced in the new archive with a change in Memento-Datetime, URI-R, or the final HTTP status code. In three cases, the HTTP status codes of mementos in the new archive change from the status codes in the original archive. \todo{WHAT THREE CASES?} Also, updating/upgrading a web archival replay tool (e.g., OpenWayback and PyWb) may affect how migrated mementos are indexed and replayed. In general, with any memento migration, we recommend that when possible requests of mementos to the original archives to be redirected to their corresponding mementos in the new archive (e.g., the case of The End of Term Archive explained above).


\subsection{National Library of Ireland}

For example, the archive Library and Archives Canada changed its domain name name from collectionscanada.gc.ca to webarchive.bac-lac.gc.ca (described in part 1), and because the archive still controls the original domain name collectionscanada.gc.ca, the archive could (even though it currently does not) redirect requests of URI-M in collectionscanada.gc.ca to the new archive webarchive.bac-lac.gc.ca. For instance, if the original archive uses the Apache web server, the mod\_rewrite rule can be used to perform automatic redirects:

\begin{lstlisting}
# With mod_rewrite
RewriteEngine on
RewriteRule   "^/webarchives/(\d{14})/(.+)" http://webarchive.bac-lac.gc.ca:8080/wayback/$1/$2  [L,R=301]
\end{lstlisting}

In the upcoming post, we will describe the movement of mementos from the Public Record Office of Northern Ireland (PRONI) web archive to Archive-It. The PRONI organization still controls and maintains the original domain name webarchive.proni.gov.uk, so it is possible for PRONI to issue redirects to the new URI-Ms in Archive-It.

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://collections.internetmemory.org/nli/content/20121223122758/http://www.whitehouse.gov/
WARC-Date: 2018-09-03T16:31:30Z
WARC-Record-ID: <urn:uuid:d03e5020-af96-11e8-9d72-f10b53f82929>

Content-Type: application/http; msgtype=response
Content-Length: 1694
HTTP/1.1 200 OK
Date: Mon, 03 Sep 2018 16:31:19 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html
Via: 1.1 varnish-v4
cache-control: max-age=86400
X-Varnish: 28318986 28187250
Memento-Datetime: Sun, 23 Dec 2012 12:27:58 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link: <http://collections.internetmemory.org/nli/content/20121223122758/http://www.whitehouse.gov/>; rel="memento"; datetime="Sun, 23 Dec 2012 12:27:58 GMT", <http://collections.internetmemory.org/nli/content/20110223072152/http://www.whitehouse.gov/>; rel="first memento"; datetime="Wed, 23 Feb 2011 07:21:52 GMT", <http://collections.internetmemory.org/nli/content/20180528183514/http://www.whitehouse.gov/>; rel="last memento"; datetime="Mon, 28 May 2018 18:35:14 GMT", <http://collections.internetmemory.org/nli/content/20121221220430/http://www.whitehouse.gov/>; rel="prev memento"; datetime="Fri, 21 Dec 2012 22:04:30 GMT", <http://collections.internetmemory.org/nli/content/20131208014833/http://www.whitehouse.gov/>; rel="next memento"; datetime="Sun, 08 Dec 2013 01:48:33 GMT", <http://collections.internetmemory.org/nli/content/timegate/http://www.whitehouse.gov/>; rel="timegate", <http://www.whitehouse.gov/>; rel="original", <http://collections.internetmemory.org/nli/content/timemap/http://www.whitehouse.gov/>; rel="timemap"; type="application/link-format"
Content-Length: 287

<HTML><head>
<title>[ARCHIVED CONTENT] Access Denied</title>
</head><BODY>
<H1>Access Denied</H1>
Reference&#32;&#35;18&#46;d8407b5c&#46;1356265678&#46;2324d94
</BODY>
</HTML>

You don't have permission to access "http&#58;&#47;&#47;wwws&#46;whitehouse&#46;gov&#47;" on this server.<P>
\end{lstlisting}

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://collections.internetmemory.org/nli/20121021203647/http://www.amazon.com/
WARC-Date: 2018-09-03T16:46:51Z
WARC-Record-ID: <urn:uuid:f4f2e910-af98-11e8-8de6-6f058c4e494a>
Content-Type: application/http; msgtype=response
Content-Length: 271841

HTTP/1.1 200 OK
Date: Mon, 03 Sep 2018 16:46:39 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html; charset=utf-8
Via: 1.1 varnish-v4
cache-control: max-age=86400
Transfer-Encoding: chunked
X-Varnish: 28349831
Memento-Datetime: Sun, 21 Oct 2012 20:36:47 GMT
Connection: keep-alive
Accept-Ranges: bytes
...
\end{lstlisting}

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://collections.internetmemory.org/nli/content/20121021203647/http://www.amazon.com/
WARC-Date: 2018-09-03T16:46:51Z
WARC-Record-ID: <urn:uuid:f500cbc0-af98-11e8-8de6-6f058c4e494a>
Content-Type: application/http; msgtype=response
Content-Length: 2642

HTTP/1.1 200 OK
Date: Mon, 03 Sep 2018 16:46:40 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html
Via: 1.1 varnish-v4
cache-control: max-age=86400
Transfer-Encoding: chunked
X-Varnish: 27227468 27453379
Memento-Datetime: Sun, 21 Oct 2012 20:36:47 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link: <http://collections.internetmemory.org/nli/content/20121021203647/http://www.amazon.com/>; rel="memento"; datetime="Sun, 21 Oct 2012 20:36:47 GMT", <http://collections.internetmemory.org/nli/content/20110221192317/http://www.amazon.com/>; rel="first memento"; datetime="Mon, 21 Feb 2011 19:23:17 GMT", <http://collections.internetmemory.org/nli/content/20180711130159/http://www.amazon.com/>; rel="last memento"; datetime="Wed, 11 Jul 2018 13:01:59 GMT", <http://collections.internetmemory.org/nli/content/20121016174254/http://www.amazon.com/>; rel="prev memento"; datetime="Tue, 16 Oct 2012 17:42:54 GMT", <http://collections.internetmemory.org/nli/content/20121025120853/http://www.amazon.com/>; rel="next memento"; datetime="Thu, 25 Oct 2012 12:08:53 GMT", <http://collections.internetmemory.org/nli/content/timegate/http://www.amazon.com/>; rel="timegate", <http://www.amazon.com/>; rel="original", <http://collections.internetmemory.org/nli/content/timemap/http://www.amazon.com/>; rel="timemap"; type="application/link-format"

<html>
<head>
<meta http-equiv="Content-Type" content="text/html;charset=iso-8859-1"/>
<title>[ARCHIVED CONTENT] 500 Service Unavailable Error</title>
</head>
<body style="padding:1% 10%;font-family:Verdana,Arial,Helvetica,sans-serif">
  <a  target="_top" href="http://collections.internetmemory.org/nli/20121021203647/http://www.amazon.com/"><img src="http://collections.internetmemory.org/nli/content/20121021203647/http://ecx.images-amazon.com/images/G/01/img09/x-site/other/a_com_logo_200x56.gif" alt="Amazon.com" width="200" height="56" border="0"/></a>
  <table>
    <tr>
      <td valign="top" style="width:52%;font-size:10pt"><br/><h2 style="color:#E47911">Oops!</h2><p>We're very sorry, but we're having trouble doing what you just asked us to do. Please give us another chance--click the Back button on your browser and try your request again. Or start from the beginning on our <a  target="_top" href="http://collections.internetmemory.org/nli/20121021203647/http://www.amazon.com/">homepage</a>.</p></td>
      <th><img src="http://collections.internetmemory.org/nli/content/20121021203647/http://ecx.images-amazon.com/images/G/01/x-locale/common/errors-alerts/product-fan-500.jpg" alt="product collage"/></th>
    </tr>
  </table>
</body>

</html>
\end{lstlisting}

\begin{lstlisting}
curl -I http://wayback.archive-it.org/10702/20121021203647/http://www.amazon.com/

HTTP/1.1 503 Service Unavailable
Server: Apache-Coyote/1.1
Content-Security-Policy-Report-Only: default-src 'self' 'unsafe-inline' 'unsafe-eval' *.archive-it.org archive-it.org *.qa-archive-it.org qa-archive-it.org archive.org *.archive.org https://*.archive-it.org https://archive-it.org https://*.qa-archive-it.org https://qa-archive-it.org https://archive.org https://*.archive.org data: blob: ; frame-src 'self' *.archive-it.org archive-it.org *.qa-archive-it.org qa-archive-it.org archive.org *.archive.org https://*.archive-it.org https://archive-it.org https://*.qa-archive-it.org https://qa-archive-it.org https://archive.org https://*.archive.org ; report-uri https://partner.archive-it.org/csp-report
Memento-Datetime: Sun, 21 Oct 2012 20:36:47 GMT
Link: <http://www.amazon.com/>; rel="original", <https://wayback.archive-it.org/10702/timemap/link/http://www.amazon.com/>; rel="timemap"; 
...
\end{lstlisting}

as the part of the WARC below shows:

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://collections.internetmemory.org/nli/20121223031837/http://www2008.org/
WARC-Date: 2018-09-03T08:40:43Z
WARC-Record-ID: <urn:uuid:0b947600-af55-11e8-9b13-5bce71cafd38>
Content-Type: application/http; msgtype=response
Content-Length: 28447

HTTP/1.1 200 OK
Date: Mon, 03 Sep 2018 08:40:30 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html; charset=utf-8
Via: 1.1 varnish-v4
cache-control: max-age=86400
Transfer-Encoding: chunked
X-Varnish: 27888670
Memento-Datetime: Sun, 23 Dec 2012 03:18:37 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link: <http://collections.internetmemory.org/nli/20121223031837/http://www2008.org/>; rel="memento"; datetime="Sun, 23 Dec 2012 03:18:37 GMT", <http://collections.internetmemory.org/nli/20121223031837/http://www2008.org/>; rel="first memento"; datetime="Sun, 23 Dec 2012 03:18:37 GMT", <http://collections.internetmemory.org/nli/20121223031837/http://www2008.org/>; rel="last memento"; datetime="Sun, 23 Dec 2012 03:18:37 GMT", <http://collections.internetmemory.org/nli/20121223031837/http://www2008.org/>; rel="prev memento"; datetime="Sun, 23 Dec 2012 03:18:37 GMT", <http://collections.internetmemory.org/nli/20121223031837/http://www2008.org/>; rel="next memento"; datetime="Sun, 23 Dec 2012 03:18:37 GMT", <http://collections.internetmemory.org/nli/timegate/http://www2008.org/>; rel="timegate", <http://www2008.org/>; rel="original", <http://collections.internetmemory.org/nli/timemap/http://www2008.org/>; rel="timemap"; type="application/link-format"



<!DOCTYPE html PUBLIC "-//W3C//DTD XHTML 1.1//EN"
...
    
\end{lstlisting}

\subsubsection{Summary}
We did not find any changes in the 979 mementos of the National Library of Ireland (NLI) collection when they were moved from europarchive.org to internetmemory.org in May 2018.  Both archives had used the same replay tool and archival banners. The NLI collection then was moved to archive-it.org in September 2018.  We found that 192 out of the 979 mementos resurfaced in archive-it.org with a change in Memento-Datetime, URI-R, or the final HTTP status code. We also found that the functionality that used to be available in the original archival banner has gone from the new archive. We also noticed that both archives internetmemory.org and archive-it.org react differently to requests of archival 4xx/5xx. 


\subsection{Public Record Office of Northern Ireland (PRONI)}

We refer to the archive from which mementos have moved as the "original archive" (i.e., PRONI archive), and we use the "new archive" to refer to the archive to which the mementos have moved (i.e., Archive-It). A memento is identified by a URI-M as defined in the Memento framework.

\paragraph{Observation 2: The functionality of the original archival banner is gone}

Similar to the archival banners provided by the European Archive and IMF, users of the PRONI archive were able to navigate through available mementos via the custom archival banner (marked in red in the top screenshot in Figure \ref{fig:proni}). Users were allowed to view the available mementos and the representation of a selected memento in the same page. Archive-It, on the other hand, uses the standard playback banner \mynote{??} (marked in red in the bottom screenshot in Figure \ref{fig:proni}). This banner does not have the same functionality compared to the original archive's banner. The new archive's banner contains information to inform users that they are viewing an ``archived" web page.

\begin{lstlisting}
$ curl --head http://wayback.archive-it.org/11112/20140408185512/http://www.www126.com/

HTTP/1.1 404 Not Found
Server: Apache-Coyote/1.1
Content-Type: text/html;charset=utf-8
Content-Length: 4910
Date: Tue, 24 Sep 2019 02:00:45 GMT
\end{lstlisting}

\begin{lstlisting}
$ curl --head --location --silent http://wayback.archive-it.org/11112/20160901021637/http://www.flickr.com/ | egrep -i "(HTTP/|^location:|^Memento-Datetime)"

HTTP/1.1 302 Found
Location: /11112/20170401014520/https://www.flickr.com/
HTTP/1.1 200 OK
Memento-Datetime: Sat, 01 Apr 2017 01:45:20 GMT
\end{lstlisting}

\begin{lstlisting}
$ curl --head --location --silent http://wayback.archive-it.org/11112/20170102004044/http://www.fws.gov/ | egrep -i "(HTTP/|^location:|^Memento-Datetime)"

HTTP/1.1 302 Found
Location: /11112/20170102004051/https://www.fws.gov/
HTTP/1.1 200 OK
Memento-Datetime: Mon, 02 Jan 2017 00:40:51 GMT
\end{lstlisting}


\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://webarchive.proni.gov.uk/20160216154000/http://www.megalithic.co.uk/
WARC-Date: 2017-11-18T03:35:22Z
WARC-Record-ID: <urn:uuid:81bb8530-cc11-11e7-9c05-ff972ac7f9f2>
Content-Type: application/http; msgtype=response
Content-Length: 60568

HTTP/1.1 200 OK
Date: Sat, 18 Nov 2017 03:35:11 GMT
Server: Apache/2.4.10
Vary: Accept-Encoding
Content-Type: text/html; charset=utf-8
Via: 1.1 varnish-v4
Memento-Datetime: Tue, 16 Feb 2016 15:40:00 GMT
...
\end{lstlisting}

\begin{lstlisting}
$ curl --head http://wayback.archive-it.org/11112/20160216154000/http://www.megalithic.co.uk/

HTTP/1.1 403 Forbidden
Server: Apache-Coyote/1.1
Content-Security-Policy-Report-Only: default-src 'self'
[...]
Memento-Datetime: Tue, 16 Feb 2016 15:40:00 GMT
X-Archive-Guessed-Charset: windows-1252
X-Archive-Orig-Server: Apache/2.2.15 (CentOS)
X-Archive-Orig-Connection: close
X-Archive-Orig-X-Powered-By: PHP/5.3.3
X-Archive-Orig-Status: 403 FORBIDDEN
X-Archive-Orig-Content-Length: 3206
X-Archive-Orig-Date: Tue, 16 Feb 2016 15:39:59 GMT
X-Archive-Orig-Warning: 199 www.megalithic.co.uk:80 You_are_abusive/hacking/spamming_www.megalithic.co.uk
X-Archive-Orig-Content-Type: text/html; charset=iso-8859-1
[...]
\end{lstlisting}

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://webarchive.proni.gov.uk/20140408185512/http://www.www126.com/
WARC-Date: 2017-11-18T02:06:22Z
WARC-Record-ID: <urn:uuid:13136370-cc05-11e7-83e9-19ddf7ecdbd2>
Content-Type: application/http; msgtype=response
Content-Length: 28657

HTTP/1.1 200 OK
Date: Sat, 18 Nov 2017 02:06:11 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html; charset=utf-8
Via: 1.1 varnish-v4
cache-control: max-age=86400
Transfer-Encoding: chunked
X-Varnish: 20429973
Memento-Datetime: Tue, 08 Apr 2014 18:55:12 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link: <http://webarchive.proni.gov.uk/20140408185512/http://www.www126.com/>; rel="memento"; datetime="Tue, 08 Apr 2014 18:55:12 GMT", <http://webarchive.proni.gov.uk/20140408185512/http://www.www126.com/>; rel="first memento"; datetime="Tue, 08 Apr 2014 18:55:12 GMT", <http://webarchive.proni.gov.uk/20140408185512/http://www.www126.com/>; rel="last memento"; datetime="Tue, 08 Apr 2014 18:55:12 GMT", <http://webarchive.proni.gov.uk/20140408185512/http://www.www126.com/>; rel="prev memento"; datetime="Tue, 08 Apr 2014 18:55:12 GMT", <http://webarchive.proni.gov.uk/20140408185512/http://www.www126.com/>; rel="next memento"; datetime="Tue, 08 Apr 2014 18:55:12 GMT", <http://webarchive.proni.gov.uk/timegate/http://www.www126.com/>; rel="timegate", <http://www.www126.com/>; rel="original", <http://webarchive.proni.gov.uk/timemap/http://www.www126.com/>; rel="timemap"; type="application/link-format"
\end{lstlisting}

\paragraph{Observation 6: PRONI may have used the Europe Archive and IMF as hosting services}

\todo{This may not need to be an observation, especially if we cite the page where it said the PRONI used Europe Archive and IMF.  Just part of the intro.}

PRONI used an archival banner that is similar to what the Europe Archive and IMF used. Furthermore, the three archives returned similar set of HTTP response headers to requests of mementos. Values of multiple response headers (e.g., server and via) are identical as shown below:

The Europe Archive:
URI-M = \url{http://collection.europarchive.org/nli/20161213111140/http://wordpress.org/}

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://collection.europarchive.org/nli/20161213111140/https://wordpress.org/
WARC-Date: 2017-12-01T18:15:32Z
WARC-Record-ID: <urn:uuid:9e705c20-d6c3-11e7-9f9e-5371622c3ef9>
Content-Type: application/http; msgtype=response
Content-Length: 159855

HTTP/1.1 200 OK
Date: Fri, 01 Dec 2017 18:15:18 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html; charset=utf-8
Via: 1.1 varnish-v4
cache-control: max-age=86400
Transfer-Encoding: chunked
X-Varnish: 15695216
Memento-Datetime: Tue, 13 Dec 2016 06:03:04 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link: ...
\end{lstlisting}

The IMF archive:
URI-M = \url{http://collections.internetmemory.org/nli/20161213111140/https://wordpress.org/}

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://collections.internetmemory.org/nli/20161213111140/https://wordpress.org/
WARC-Date: 2018-09-03T16:33:41Z
WARC-Record-ID: <urn:uuid:1e3173c0-af97-11e8-8819-6df9b412b877>
Content-Type: application/http; msgtype=response
Content-Length: 300060

HTTP/1.1 200 OK
Date: Mon, 03 Sep 2018 16:33:27 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html; charset=utf-8
Via: 1.1 varnish-v4
cache-control: max-age=86400
Transfer-Encoding: chunked
X-Varnish: 11721161
Memento-Datetime: Tue, 13 Dec 2016 06:03:04 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link:...
\end{lstlisting}

The PRONI archive:
URI-M = \url{http://webarchive.proni.gov.uk/20100218151844/http://www.berr.gov.uk/}

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://webarchive.proni.gov.uk/20100218151844/http://www.berr.gov.uk/
WARC-Date: 2017-12-01T01:59:56Z
WARC-Record-ID: <urn:uuid:5452da60-d63b-11e7-91e2-8bf9abaf94b4>
Content-Type: application/http; msgtype=response
Content-Length: 36908

HTTP/1.1 200 OK
Date: Fri, 01 Dec 2017 01:59:43 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html; charset=utf-8
Via: 1.1 varnish-v4
cache-control: max-age=86400
Transfer-Encoding: chunked
X-Varnish: 16262557
Memento-Datetime: Thu, 18 Feb 2010 15:18:44 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link: ...
\end{lstlisting}

We found that PRONI archival collection was listed as one of the maintained collections by the Europe Archive and IMF.

Even though the PRONI collection was moved from the Europe Archive to IMF, URI-Ms served by \url{proni.gov.uk} had not changed. It is possible that the PRONI archive followed a strategy of serving mementos under \url{proni.gov.uk} while using the hosting services provided by the Europe Archive and IMF. Thus, the regular users of the PRONI archive did not notice any change in URI-Ms. We do not think custom domains are available with Archive-It, so PRONI was unable to continue to host their mementos in their own URI namespace.

\begin{lstlisting}
WARC/1.0
WARC-Type: response
WARC-Target-URI: http://webarchive.proni.gov.uk/content/20160216154000/http://www.megalithic.co.uk/
WARC-Date: 2017-11-18T03:35:22Z
WARC-Record-ID: <urn:uuid:81c967e0-cc11-11e7-9c05-ff972ac7f9f2>
Content-Type: application/http; msgtype=response
Content-Length: 4587

HTTP/1.1 200 OK
Date: Sat, 18 Nov 2017 03:35:11 GMT
Server: Apache/2.4.10
Age: 0
Vary: Accept-Encoding
Content-Type: text/html
Via: 1.1 varnish-v4
cache-control: max-age=86400
X-Varnish: 24849777 24360264
Memento-Datetime: Tue, 16 Feb 2016 15:40:00 GMT
Connection: keep-alive
Accept-Ranges: bytes
Link: ...

<html>
<head>
<META NAME="ROBOTS" CONTENT="NOINDEX, NOFOLLOW">
<title>[ARCHIVED CONTENT] 403 FORBIDDEN : LOGGED BY www.megalithic.co.uk</title>
</head>
<body style=\"font:Arial Black,Arial\">
<p><b><font color="#FF0000" size="+2" face="Verdana, Arial, Helvetica, sans-serif" style="text-decoration:blink; color:#FF0000; background:#000000;">&nbsp;&nbsp;&nbsp;&nbsp; 403 FORBIDDEN! &nbsp;&nbsp;&nbsp;&nbsp;</font></b></p>
<b>
<p><font color="#FF0000">You have been blocked from the Megalithic Portal by our defence robot.<br>Possibly the IP address you are accessing from has been banned for previous bad behavior or you have attempted a hostile action.<br>If you think this is an error please click the Trouble Ticket link below to communicate with the site admin.</font></p>
...
\end{lstlisting}

\subsubsection{Summary}
We described the movement of mementos from the PRONI archive (proni.gov.uk) to archive-it.org in October 2018. We found that 114 out of the 469 mementos resurfaced in archive-it.org with a change in Memento-Datetime, URI-R, or the final HTTP status code. We also found that the functionality that used to be available in the original archival banner has gone. We noticed that both archives proni.gov.uk and archive-it.org react differently to requests of archival 4xx/5xx. 

\subsection{WebCite}

\url{https://ws-dl.blogspot.com/2019/10/2019-10-21-where-did-archive-go-part-4.html}

In the last part of this four part series, we focus on changes in webcitation.org (WebCite). The WebCite archive has been operational in its current form since at least 2004 and was the first archive to offer an on-demand archiving service by allowing users to submit URLs of web pages. Around 2019-06-07, the archive became unreachable. The Wayback Machine indicates that there were no mementos captured for the domain webcitation.org between 2019-06-07 and 2019-07-09 (for about a month), which is the longest period of time in 2019 that has no mementos for WebCite in the Internet Archive:

The host webcitation.org was not resolving as shown in the cURL session below:

\begin{lstlisting}
$ date
Mon Jul 01 01:33:15 EDT 2019

$ curl -I www.webcitation.org
curl: (6) Could not resolve host: www.webcitation.org
\end{lstlisting}

We were conducting a study on a set of mementos from WebCite when the archive was inaccessible. The study included downloading the mementos and storing them locally in WARC files. Because the archive was unreachable, the WARC files contained only request records, with no response records, as shown below (the URI of the memento (URI-M) was \url{http://www.webcitation.org/5ekDHBAVN}):

\begin{lstlisting}
WARC/1.0
WARC-Type: request
WARC-Target-URI: http://www.webcitation.org/5ekDHBAVN
WARC-Date: 2019-07-09T02:01:52Z
WARC-Concurrent-To: <urn:uuid:8519ea60-a1ed-11e9-82a3-4d5f15d9881d>
WARC-Record-ID: <urn:uuid:851c5b60-a1ed-11e9-82a3-4d5f15d9881d>
Content-Type: application/http; msgtype=request
Content-Length: 303

GET /5ekDHBAVN HTTP/1.1
Upgrade-Insecure-Requests: 1
User-Agent: Web Science and Digital Libraries Group (@WebSciDL); Project/archives_fixity; Contact/Mohamed Aturban (maturban@odu.edu)
X-DevTools-Emulate-Network-Conditions-Client-Id: 5B0BDCB102052B8A7EF0772D50B85540
Host: www.webcitation.org

<EOF>
\end{lstlisting}
 
The WebCite archive was back online on 2019-07-09 with a significant change; the archive no longer accepts archiving requests as its homepage indicates (e.g., the first screenshot above). 

Our WARC records below show the time at which the archive came back online on 2019-07-09T13:17:16Z. Note that there are a few hours difference between the value of the WARC-Date below and its value in the WARC record above. However, the WebCite archive was still down on 2019-07-09T02:01:52Z,  while it was online again around 13:17:16Z:

\begin{lstlisting}
WARC/1.0
WARC-Type: request
WARC-Target-URI: http://www.webcitation.org/6MIxPlJUQ
WARC-Date: 2019-07-09T13:17:16Z
WARC-Concurrent-To: <urn:uuid:df5de3b0-a24b-11e9-aaf9-bb34816ea2ff>
WARC-Record-ID: <urn:uuid:df5f6a50-a24b-11e9-aaf9-bb34816ea2ff>
Content-Type: application/http; msgtype=request
Content-Length: 414

GET /6MIxPlJUQ HTTP/1.1
Pragma: no-cache
Accept-Encoding: gzip, deflate
Host: www.webcitation.org
Upgrade-Insecure-Requests: 1
User-Agent: Web Science and Digital Libraries Group (@WebSciDL); Project/archives_fixity; Contact/Mohamed Aturban (maturban@odu.edu)
Accept: text/html,application/xhtml+xml,application/xml;q=0.9,image/webp,image/apng,*/*;q=0.8
Cache-Control: no-cache
Connection: keep-alive

WARC/1.0
WARC-Type: response
WARC-Target-URI: http://www.webcitation.org/6MIxPlJUQ
WARC-Date: 2019-07-09T13:17:16Z
WARC-Record-ID: <urn:uuid:df5fb870-a24b-11e9-aaf9-bb34816ea2ff>
Content-Type: application/http; msgtype=response
Content-Length: 1212

HTTP/1.1 200 OK
Pragma: no-cache
Date: Tue, 09 Jul 2019 13:16:47 GMT
Server: Apache/2.4.29 (Ubuntu)
Vary: Accept-Encoding
Content-Type: text/html; charset=UTF-8
Set-Cookie: PHPSESSID=ugssainrn4pne801m58d41lm2r; path=/
Cache-Control: no-store, no-cache, must-revalidate
Connection: Keep-Alive
Keep-Alive: timeout=5, max=100
Content-Length: 814
Expires: Thu, 19 Nov 1981 08:52:00 GMT

<!DOCTYPE html PUBLIC
...
The archive was still down a few seconds before 2019-07- 09T13:17:16Z as there were not response records in the WARC files:

WARC/1.0
WARC-Type: request
WARC-Target-URI: http://www.webcitation.org/6E2fTSO15
WARC-Date: 2019-07-09T13:16:39Z
WARC-Concurrent-To: <urn:uuid:c94dd940-a24b-11e9-8d2f-a5805b26a392>
WARC-Record-ID: <urn:uuid:c9515bb0-a24b-11e9-8d2f-a5805b26a392>
Content-Type: application/http; msgtype=request
Content-Length: 303

GET /6E2fTSO15 HTTP/1.1
Upgrade-Insecure-Requests: 1
User-Agent: Web Science and Digital Libraries Group (@WebSciDL); Project/archives_fixity; Contact/Mohamed Aturban (maturban@odu.edu)
X-DevTools-Emulate-Network-Conditions-Client-Id: 78DDE3B763F42A09787D0EBA241C9C4A
Host: www.webcitation.org
\end{lstlisting}

The archive has had some issues in the past related to funding limitations:

\begin{lstlisting}
#WebCite will stop accepting new submissions end of 2013, unless they reach their fundraising goals http://t.co/nug32Zzc . Please support.
- Ahmed AlSum (@aalsum) February 16, 2013
\end{lstlisting}

One of the main objectives for which WebCite was established was to reduce the impact of reference rot by allowing researchers and authors of scientific work to archive cited web pages. The instability in providing archiving services and being inaccessible from time to time raises important questions:

Is there any plan by the web archiving community to recover web pages archived by WebCite if the archive is gone? 
Why didn't the archive give a notice (e.g., in their homepage) before they became unreachable? This will give users some time to deal with different scenarios, such as downloading a particular set of mementos
Has the archived content changed before the archive came back online?
The archive now does not accept archiving requests nor does it do web page crawling. Is there any plan by the archive to resume the on-demand archiving service in the future?
In case WebCite disappears, the structure of the URI-M used by the archive makes it difficult to recover mementos from other web archives. This is because the URI-M of a memento (e.g., \url{www.webcitation.org/5BmjfFFB1}) does not give any additional information about the memento. These shortened URI-Ms are also used by other archives, such as archive.is and perma.cc. In contrast, the majority of web archives that employ one of the Wayback Machine’s implementations (e.g., OpenWayback and PyWb) use the URI-M structure illustrated below. Note that archive.is and perma.cc also support this Wayback Machine-style URI-Ms (i.e., each memento has two URI-Ms):

This common URI-M structure provides two pieces of information, the original page's URI (URI-R) and the creation datetime of the memento (Memento-Datetime). This information then can be used to look up similar (or even identical) archived pages in other web archives using services like the LANL Memento aggregator. With the URI-M structure used by WebCite, it is not possible to recover mementos using only the URI-M. The Robust Links article introduces a mechanism to allow a user to link to an original URI and at the same time describe the state of the URI so that, in the future, users will be able to obtain information about the URI even if it disappears from the live web.

The WebCite archive is a well-known web archive and one of the few on-demand archiving services. It is important that the web archiving community takes further steps to guarantee long-term preservation and stability of those archived pages at webcitation.org. 


\section{Perma.cc}

\begin{enumerate}
\footnotesize
\item \url{http://perma-archives.org/warc/20170731024959/https://www.tmall.com/}
\item \url{http://perma-archives.org/warc/20170203233757/https://www.cms.gov/cciio/index.html}
\item \url{http://perma-archives.org/warc/20141021173834/http://databank.worldbank.org/data/home.aspx}
\item \url{http://perma-archives.org/warc/20151101192051/http://www.homedepot.com/}
\item \url{http://perma-archives.org/warc/20161118165253/https://studentloans.gov/myDirectLoan/index.action}
\item \url{http://perma-archives.org/warc/20151009235521/http://readwrite.com/}
\item \url{http://perma-archives.org/warc/20160914003340/https://www.texas.gov/}
\item \url{http://perma-archives.org/warc/20170220021805/https://www.sam.gov/portal/SAM/}
\item \url{http://perma-archives.org/warc/20151101193342/http://www.spiegel.de/}
\item \url{http://perma-archives.org/warc/20150404172754/https://www.att.com/}
\item \url{http://perma-archives.org/warc/20150820154813/http://ici.radio-canada.ca/}
\item \url{http://perma-archives.org/warc/20170925035325/https://www.dropbox.com/?landing=dbv2}
\item \url{http://perma-archives.org/warc/20161105175946/http://www.hostgator.com/}
\item \url{http://perma-archives.org/warc/20150123144122/http://www.usa.gov/page-not-found}
\item \url{http://perma-archives.org/warc/20151002194849/http://eric.ed.gov/}
\item \url{http://perma-archives.org/warc/20160204202605/https://www.icloud.com/}
\item \url{http://perma-archives.org/warc/20171003185440/https://travel.state.gov/content/travel/en/404.html}
\item \url{http://perma-archives.org/warc/20171022230759/https://www.consumer.ftc.gov/}
\end{enumerate}


\begin{lstlisting}
$ curl -i https://perma.cc/timemap/link/https://www.consumer.ftc.gov/

HTTP/1.1 404 Not Found
Date: Tue, 20 Apr 2021 08:34:01 GMT
Content-Type: text/html; charset=utf-8
Transfer-Encoding: chunked
Connection: keep-alive
Set-Cookie: __cfduid=d9155b0a0966cf8be393cdae6f8204d031618907641; expires=Thu, 20-May-21 08:34:01 GMT; path=/; domain=.perma.cc; HttpOnly; SameSite=Lax; Secure
X-Memento-Count: 0
Cache-Control: max-age=1800
X-Frame-Options: DENY
Vary: Cookie, Host
CF-Cache-Status: DYNAMIC
cf-request-id: 0990034f690000617df9053000000001
Expect-CT: max-age=604800, report-uri="https://report-uri.cloudflare.com/cdn-cgi/beacon/expect-ct"
Set-Cookie: __cflb=0H28vJJdLkHc3TMWQrwoPYCkNvS1ueQqP9XurCxvVQ8; SameSite=None; Secure; path=/; expires=Wed, 21-Apr-21 07:34:01 GMT; HttpOnly
Server: cloudflare
CF-RAY: 642d07f8af38617d-ORD

404 page not found
\end{lstlisting}

